CoGenesis: A Framework Collaborating Large and Small Language Models for Secure Context-Aware Instruction Following

With the advancement of language models (LMs), their exposure to private data is increasingly inevitable, and their deployment (especially for smaller ones) on personal devices, such as PCs and smartphones, has become a prevailing trend. In contexts laden with user information, enabling models to both safeguard user privacy and execute commands efficiently emerges as an essential research imperative. In this paper, we propose CoGenesis, a collaborative generation framework integrating large (hosted on cloud infrastructure) and small models (deployed on local devices) to address privacy concerns logically. Initially, we design a pipeline to create personalized writing instruction datasets enriched with extensive context details as the testbed of this research issue. Subsequently, we introduce two variants of CoGenesis based on sketch and logits respectively. Our experimental findings, based on our synthesized dataset and two additional open-source datasets, indicate that: 1) Large-scale models perform well when provided with user context but struggle in the absence of such context. 2) While specialized smaller models fine-tuned on the synthetic dataset show promise, they still lag behind their larger counterparts. 3) Our CoGenesis framework, utilizing mixed-scale models, showcases competitive performance, providing a feasible solution to privacy issues.

==> ack.tex <==
\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> table-auto.tex <==
\begin{table*}[ht]
  \small
  \centering
  \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{lllllllllll}
    \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{Params} & \multicolumn{3}{c}{Context-aware Instructions} & \multicolumn{3}{c}{Avocado Emails} & \multicolumn{3}{c}{Academic Paper Abstracts} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} 
                        &       & Ovl.(w) & Per. & Ovl.(w/o) & Ovl.(w) & Per. & Ovl.(w/o) & Ovl.(w) & Per. &  Ovl.(w/o)  \\
    \midrule
    \multicolumn{11}{l}{ \quad \quad \textbf{\textit{zero-shot LLM with context (upper bound)}}} \\
     L1 GPT-4-turbo     & N/A   &  \textbf{8.85}  &  \textbf{8.90}  &  \textbf{8.54}  &  \textbf{8.31}  &  \textbf{7.71}  &  \textbf{8.05}  &  \textbf{8.64}  &  \textbf{8.47}  &  \textbf{8.68} \\
     L2 GPT-3.5-turbo   & N/A   &  8.30  &  8.33  &  7.58  &  7.70  &  7.45  &  7.57  &  7.97  &  7.88  &  8.29 \\
     L3 Llama-2-Chat    & 70B   &  7.78  &  7.98  &  7.96  &  7.00  &  7.18  &  \underline{8.05}  &  7.48  &  7.12  &  8.32 \\
     L4 Qwen-Chat(v1)   & 72B   &  8.38  &  8.38  &  8.14  &  7.62  &  7.10  &  7.70  &  7.90  &  7.62  &  8.24 \\
     L5 Qwen-Chat(v1.5) & 72B   &  \underline{8.70}  &  \underline{8.67}  &  \underline{8.26}  &  \underline{8.20}  &  \underline{7.69}  &  7.80  &  \underline{8.52}  &  \underline{8.16}  &  \underline{8.60} \\
     L6 Mixtral-8x7b    & 47B   &  8.12  &  8.22  &  7.96  &  7.35  &  6.88  &  6.92  &  7.92  &  7.62  &  8.08 \\
     \midrule
     \midrule
     \multicolumn{11}{l}{ \quad \quad \textbf{\textit{zero-shot LLM w/o context (lower bound)}}} \\
     L1 GPT-4-turbo     & N/A   &  \textbf{6.10}  &  \textbf{6.46}  &  \textbf{8.75}  &  \underline{5.10}  &  \underline{3.79}  &  \textbf{8.58}  &  \textbf{8.42}  &  \textbf{7.94}  &  \textbf{8.73} \\
     L2 GPT-3.5-turbo   & N/A   &  4.34  &  3.76  &  7.47  &  3.72  &  3.03  &  7.61  &  3.37  &  3.59  &  6.04 \\
     L3 Llama-2-Chat    & 70B   &  4.74  &  4.60  &  8.12  &  3.38  &  3.52  &  8.04  &  6.74  &  6.18  &  7.90 \\
     L4 Qwen-Chat(v1)   & 72B   &  3.70  &  3.38  &  7.72  &  3.28  &  2.38  &  7.50  &  6.42  &  5.54  &  7.90 \\
     L5 Qwen-Chat(v1.5) & 72B   &  \underline{5.86}  &  \underline{5.98}  &  \underline{8.52}  &  \textbf{5.83}  &  \textbf{4.40}  &  \underline{8.54}  &  \underline{7.92}  &  \underline{7.16}  &  \underline{8.28} \\
     L6 Mixtral-8x7b    & 47B   &  5.32  &  5.08  &  8.14  &  3.38  &  3.52  &  8.04  &  6.74  &  6.18  &  7.90 \\
     \midrule
     \midrule
     \multicolumn{11}{l}{ \quad \quad \textbf{\textit{zero-shot SLM with context}}} \\
     S1 StableLM-Zephyr &  1.6B &  \textbf{6.88}  &  6.82  &  \underline{6.68}  &  \textbf{6.03}  &  \textbf{5.49}  &  \underline{6.51}  &  \textbf{7.32}  &  \textbf{6.94}  &  \textbf{8.14} \\
     S2 H2O-danube-chat &  1.8B &  6.56  &  \textbf{6.94}  &  6.60  &  4.77  &  \underline{5.00}  &  \textbf{6.57}  &  5.98  &  5.54  &  6.94 \\
     S3 TinyLlama-Chat  &  1.1B &  1.72  &  1.84  &  2.14  &  4.00  &  3.54  &  5.40  &  1.96  &  1.88  &  4.24 \\
     S4 Qwen-Chat(v1)   &  1.8B &  5.78  &  5.50  &  6.00  &  4.91  &  4.54  &  6.49  &  4.46  &  5.04  &  6.74 \\
     S5 Qwen-Chat(v1.5) &  1.8B &  \underline{6.86}  &  \underline{6.86}  &  \textbf{7.20}  &  \underline{5.51}  &  4.89  &  6.14  &  \underline{6.42}  &  \underline{6.14}  &  \underline{7.78} \\
     \midrule
     \midrule
     \multicolumn{11}{l}{ \quad \quad \textbf{\textit{finetuned SLM (+ LLM) with context}}} \\
     S1 StableLM-Zephyr 
                    &  1.6B &  8.30 &  8.56  &  7.73  &  7.58  &  6.70  &  7.20  &  7.96  &  7.64  &  8.18 \\
     \quad \quad \textit{+ L1 sketch}
                    & \textit{mixed}  &  8.48\textcolor{red}{$_{\uparrow 0.18}$} &  8.56\textcolor{red}{$_{\uparrow 0.00}$}  &  7.98\textcolor{red}{$_{\uparrow 0.25}$}  &  7.68\textcolor{red}{$_{\uparrow 0.10}$}  &  6.62\textcolor{blue}{$_{\downarrow 0.08}$}  &  7.48\textcolor{red}{$_{\uparrow 0.28}$}  &  8.28\textcolor{red}{$_{\uparrow 0.32}$}  &  7.48\textcolor{blue}{$_{\downarrow 0.16}$}  &  8.38\textcolor{red}{$_{\uparrow 0.20}$} \\ \midrule
     S2 H2O-danube-chat 
                    &  1.8B &  7.64 &  7.58  &  7.00  &  6.50  &  6.16  &  6.34  &  7.70  &  7.30  &  8.06 \\
     \quad \quad \textit{+ L1 sketch}
                    & \textit{mixed}  &  7.84\textcolor{red}{$_{\uparrow 0.20}$} &  7.78\textcolor{red}{$_{\uparrow 0.20}$}  &  7.14\textcolor{red}{$_{\uparrow 0.14}$}  &  7.14\textcolor{red}{$_{\uparrow 0.64}$}  &  6.72\textcolor{red}{$_{\uparrow 0.56}$}  &  7.52\textcolor{red}{$_{\uparrow 1.18}$}  &  8.10\textcolor{red}{$_{\uparrow 0.40}$}  &  7.28\textcolor{blue}{$_{\downarrow 0.02}$}  &  8.18\textcolor{red}{$_{\uparrow 0.12}$} \\ \midrule
     S3 TinyLlama-Chat  
                    &  1.1B &  7.42 &  7.66  &  6.78  &  6.12  &  5.92  &  6.20  &  7.66  &  7.32  &  8.18 \\
     \quad \quad \textit{+ L1 sketch}
                    & \textit{mixed}  &  7.66\textcolor{red}{$_{\uparrow 0.24}$} &  7.14\textcolor{blue}{$_{\downarrow 0.52}$}  &  6.82\textcolor{red}{$_{\uparrow 0.04}$}  &  6.58\textcolor{red}{$_{\uparrow 0.46}$}  &  6.02\textcolor{red}{$_{\uparrow 0.10}$}  &  6.60\textcolor{red}{$_{\uparrow 0.40}$}  &  7.72\textcolor{red}{$_{\uparrow 0.06}$}  &  7.36\textcolor{red}{$_{\uparrow 0.04}$}  &  8.10\textcolor{blue}{$_{\downarrow 0.08}$} \\
     \quad \quad \textit{+ L3 logits}
                    & \textit{mixed}  &  7.76\textcolor{red}{$_{\uparrow 0.34}$}  &  7.74\textcolor{red}{$_{\uparrow 0.08}$}  &  7.06\textcolor{red}{$_{\uparrow 0.28}$}  &   6.06\textcolor{blue}{$_{\downarrow 0.06}$}  &  6.16\textcolor{red}{$_{\uparrow 0.24}$}  &  6.94\textcolor{red}{$_{\uparrow 0.74}$}  &  8.14\textcolor{red}{$_{\uparrow 0.48}$}  &  7.34\textcolor{red}{$_{\uparrow 0.02}$}   &  8.04\textcolor{blue}{$_{\downarrow 0.14}$}  \\ \midrule
     S4 Qwen-Chat(v1)   
                    &  1.8B &  7.44 &  7.76  &  7.02  &  7.00  &  6.71  &  7.06  &  7.84  &  7.36  &  8.18 \\
     \quad \quad \textit{+ L1 sketch}
                    & \textit{mixed}  &  7.80\textcolor{red}{$_{\uparrow 0.36}$} &  7.82\textcolor{red}{$_{\uparrow 0.06}$}  &  7.64\textcolor{red}{$_{\uparrow 0.62}$}  &  7.18\textcolor{red}{$_{\uparrow 0.18}$}  &  6.44\textcolor{blue}{$_{\downarrow 0.27}$}  &  7.28\textcolor{red}{$_{\uparrow 0.22}$}  &  8.02\textcolor{red}{$_{\uparrow 0.18}$}  &  7.70\textcolor{red}{$_{\uparrow 0.34}$}  &  8.34\textcolor{red}{$_{\uparrow 0.16}$} \\
     \quad \quad \textit{+ L4 logits}
                    & \textit{mixed}  &  8.12\textcolor{red}{$_{\uparrow 0.68}$} &  8.20\textcolor{red}{$_{\uparrow 0.44}$}  &  7.86\textcolor{red}{$_{\uparrow 0.84}$}  &  7.48\textcolor{red}{$_{\uparrow 0.48}$}  &  6.44\textcolor{blue}{$_{\downarrow 0.27}$}  &  7.46\textcolor{red}{$_{\uparrow 0.40}$}  &  7.92\textcolor{red}{$_{\uparrow 0.08}$}  &  7.16\textcolor{blue}{$_{\downarrow 0.20}$}      &  8.30\textcolor{red}{$_{\uparrow 0.12}$}  \\ \midrule
     S5 Qwen-Chat(v1.5)
                    &  1.8B &  8.08 &  8.12  &  7.40  &  6.34  &  5.56  &  6.54  &  7.68  &  7.30  &  8.18 \\
     \quad \quad \textit{+ L1 sketch}
                    & \textit{mixed}  &  8.18\textcolor{red}{$_{\uparrow 0.10}$} &  7.98\textcolor{blue}{$_{\downarrow 0.14}$}  &  7.62\textcolor{red}{$_{\uparrow 0.22}$}  &  6.54\textcolor{red}{$_{\uparrow 0.20}$}  &  5.84\textcolor{red}{$_{\uparrow 0.28}$}  &  6.74\textcolor{red}{$_{\uparrow 0.20}$}  &  8.10\textcolor{red}{$_{\uparrow 0.42}$}  &  7.24\textcolor{blue}{$_{\downarrow 0.06}$}  &  8.32\textcolor{red}{$_{\uparrow 0.14}$} \\
     \quad \quad \textit{+ L5 logits}
                    & \textit{mixed} & 8.28\textcolor{red}{$_{\uparrow 0.20}$}  &  8.22\textcolor{red}{$_{\uparrow 0.10}$}  &  7.80\textcolor{red}{$_{\uparrow 0.40}$}  &   6.66\textcolor{red}{$_{\uparrow 0.32}$} & 5.70\textcolor{red}{$_{\uparrow 0.14}$} &  7.12\textcolor{red}{$_{\uparrow 0.58}$} & 8.14\textcolor{red}{$_{\uparrow 0.46}$} & 7.28\textcolor{blue}{$_{\downarrow 0.02}$} & 8.40\textcolor{red}{$_{\uparrow 0.22}$} \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{
    The table displays the performance of LLMs and SLMs in both \textit{with context} and \textit{w/o context} settings. We highlight the best result in \textbf{bold}, the second in \underline{underline} and indicate variations in each SLM using \textcolor{red}{$\uparrow$} and \textcolor{blue}{$\downarrow$}.
  }
  \label{tab:main_results}
\end{table*}


==> table-human.tex <==
\begin{table*}[ht]
  \small
  \centering
  \scalebox{0.85}{
  \begin{tabular}{clllllllll}
    \toprule
    \midrule
     \multirow{2}{*}{Category} & \multirow{2}{*}{Model} & ChatGPT & \multicolumn{5}{c}{Human Eval}  & \multicolumn{2}{c}{Avg Coefficient} \\
    \cmidrule(lr){4-8} \cmidrule(lr){9-10} 
     & &  Eval.Avg  &  Novelty & Relevance & Significance & Verifiability & Avg & Pearson & Spearman \\
    \midrule
     \multirow{2}{*}{API-based} 
     & gpt-3.5-turbo(0-shot)    &  1.90  &  1.54  &  2.69  &  1.77  &  2.08  &  2.02  &  0.87  &  0.78 \\
     & gpt-3.5-turbo(5-shot)*   &  1.96  &  1.31  &  2.62  &  2.08  &  2.62  &  2.15  &  0.80  &  0.78 \\
     \midrule
     \multirow{5}{*}{General} 
     & Llama-2-70b-chat(0-shot) &  2.04  &  1.77  &  2.23  &  1.92  &  1.92  &  1.96  &  0.89  &  0.84 \\
     & Llama-2-70b-chat(5-shot) &  2.20  &  2.15  &  2.77  &  2.08  &  2.31  &  2.33  &  0.96  &  0.90 \\
     & Llama-2-70b-chat(5-shot)*&  2.01  &  1.38  &  2.62  &  2.31  &  2.00  &  2.08  &  0.97  &  0.94 \\
     & WizardLM-70B-V1.0(0-shot)&  1.91  &  1.38  &  2.31  &  1.54  &  2.00  &  1.81  &  0.90  &  0.75 \\
     & WizardLM-70B-V1.0(5-shot)&  2.01  &  1.15  &  2.69  &  2.46  &  1.77  &  2.02  &  0.85  &  0.89 \\
     \midrule
     \multirow{2}{*}{Medicine} 
     & PMC-LLaMA-13B(0-shot)    &  1.41  &  1.00  &  2.62  &  1.92  &  2.00  &  1.88  &  0.73  &  0.73 \\
     & PMC-LLaMA-13B(5-shot)*   &  1.97  &  1.85  &  2.23  &  1.92  &  1.69  &  1.92  &  0.95  &  0.94 \\
     \midrule
     SFT & WizardLM-13BV1.2     &  1.79  &  0.85  &  2.77  &  1.23  &  2.23  &  1.77  &  0.83  &  0.85 \\
     \midrule
    \bottomrule
  \end{tabular}}
  \caption{
  This table presents the results of human evaluation. The \textit{Avg Coefficient} are used to assess the correlation between the average scores obtained from ChatGPT and human.
  }
  \label{tab:human_eval}
\end{table*}

